Automatic Snake Gait Generation Using Model Predictive Control

In this paper, we propose a method for generating undulatory gaits for snake robots. Instead of starting from a pre-defined movement pattern such as a serpenoid curve, we use a Model Predictive Control approach to automatically generate effective locomotion gaits via trajectory optimization. An important advantage of this approach is that the resulting gaits are automatically adapted to the environment that is being modeled as part of the snake dynamics. To illustrate this, we use a novel model for anisotropic dry friction, along with existing models for viscous friction and fluid dynamic effects such as drag and added mass. For each of these models, gaits generated without any change in the method or its parameters are as efficient as Pareto-optimal serpenoid gaits tuned individually for each environment. Furthermore, the proposed method can also produce more complex or irregular gaits, e.g. for obstacle avoidance or executing sharp turns.

==> Makefile <==
DIR := $(shell pwd)
PAPER := icra2020_snake_locomotion

paper:
	pdflatex -output-directory pdf --jobname=$(PAPER) ms.tex; \
	bibtex pdf/$(PAPER).aux; \
	pdflatex -output-directory pdf --jobname=$(PAPER) ms.tex; \
	pdflatex -output-directory pdf --jobname=$(PAPER) ms.tex; \

clean:
	rm -f pdf/*; \
	rm -f *.bbl; \
	rm -f $(PAPER)_arxiv.tgz; \

arxiv: paper
	rm -f $(PAPER)_arxiv.tgz; \
	touch $(PAPER)_arxiv.tgz; \
	cp pdf/$(PAPER).bbl ./ms.bbl; \
	tar --exclude=$(PAPER)_arxiv.tgz -cvzf $(PAPER)_arxiv.tgz --exclude-vcs --exclude=extra --exclude=download --exclude=bib --exclude=pdf --exclude=Makefile --exclude=*~ .

all: paper


==> baselines.tex <==
\section{Baselines}\label{sec:baselines}

To evaluate our MPC-based gait generation approach, we introduce a baseline of gaits created by serpenoid curves. For each joint, the desired angle $\phi_i$ follows the serpenoid curve
\begin{equation}
\phi_i(t)=\alpha sin(2\pi ft + (i-1)\beta) + \gamma \label{serpenoid_curve}
\end{equation}
where $f$, $\beta$ and $\gamma$ are the parameters to be designed for the snake gaits. PID controllers are used for joint position control.
To perform an optimal search, we apply grid search over the gait parameters and PID controllers. We use the resulting gaits to find the Pareto-optimal front \cite{belegundu2019optimization} giving the best tradeoff between power consumption and locomotion speed. 
